Compiling a Higher-Order Smart Contract Language to LLVM

Scilla is a higher-order polymorphic typed intermediate level language for implementing smart contracts. In this talk, we describe a Scilla compiler targeting LLVM, with a focus on mapping Scilla types, values, and its functional language constructs to LLVM-IR. The compiled LLVM-IR, when executed with LLVM's JIT framework, achieves a speedup of about 10x over the reference interpreter on a typical Scilla contract. This reduced latency is crucial in the setting of blockchains, where smart contracts are executed as parts of transactions, to achieve peak transactions processed per second. Experiments on the Ackermann function achieved a speedup of more than 45x. This talk abstract is aimed at both programming language researchers looking to implement an LLVM based compiler for their functional language, as well as at LLVM practitioners.

==> Makefile <==

all: paper.pdf

quick: Makefile *.tex *.bib *.cls
	pdflatex paper

paper.pdf: Makefile *.tex *.bib *.cls
	pdflatex paper
	bibtex paper -min-crossrefs=5
	pdflatex paper
	pdflatex paper

ext:
	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"
	bibtex paper-extended -min-crossrefs=5
	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"
	pdflatex --jobname=paper-extended "\def\extflag{}\input{paper}"

clean:
	rm -f *.aux *.bbl *.blg *.log *.out *.rel paper.pdf cover.pdf

diff:
	cd ../diff; make; cd ../current

zip:
	zip paper.zip Makefile *.tex *.bib *.cls plots/*.pdf


cover: cover.tex
	pdflatex cover
	pdflatex cover

.PHONY: all clean *.tex *.bib *.cls


==> fig-llvmdev-domain.tex <==
{\small{
$
\begin{array}{l@{\ \ }r@{\ \ }c@{\ \ }l}
%
%
\text{(Variable environment)}
& \venv & \in & \Var \pfun \subsets{\Expr}
\\[1pt]
\text{(Type environment)}
& \tenv & \in & \TVar \pfun \subsets{\Type}
\\[1pt]
\text{(Label environment)}
& \cenv & \in & \Labs \pfun \subsets{\Expr}
\\[1pt]
\end{array}
$
}}  


==> fig-llvmdev-rules.tex <==
\footnotesize{
\begin{mathpar}
%
%
% Let
\inferrule*
{
\tenv, \venv, \lenv \vDash \lenv(\lab{1}) \subseteq \venv(x) 
\\
\tenv, \venv, \lenv \vDash \labe{1}
\\
\tenv, \venv, \lenv \vDash \labe{2}
}
{\tenv, \venv, \lenv \vDash \Let{x}{\labe{1}}{\labe{2}}}
%
%
% \and
% \vspace{-5pt}
% %
% %
% % Functions
% \inferrule*
% {\senv, \ident : \gatom \vdash \expr \hassig \angled{\many{\ident_j}; s; g}}
% {\senv \vdash \Fun{\ident}{\typ}{\expr} \hassig \angled{\ident, \many{\ident_j}; s; g}}
% %
% %
% \and
% %
% % Application
% \inferrule*[width=15em]
% {
% \senv \vdash \ident \hassig \vsig \\
% \forall j, \senv \vdash \ident_j \hassig \vsig_j \\
% \vsig' = \applySig (\vsig, \vsig_j)
% }
% {\senv \vdash \ident,~\many{\ident_j} \hassig \vsig' }
% %
% %
% \and
% %
% %
% \applySig\ \vsig\ \many{\vsig_j} =
% \begin{cases}
%   \angled{[], \gusapp\ \ident\ \many{\ident_j}, \gugapp~\ident~\many{\ident_j}} & \text{if}~\vsig = \tp{atom} \\
%   \angled{[], [\many{(\text{size}~\vsig_j)} / \many{\ident_j}]s, [\many{(\text{gas}~\vsig_j)} /
%     \many{\ident_j}] g} & \text{if}~\vsig = \angled{\many{\ident_j},
%     s, g}
% \end{cases}
%
%
%
\end{mathpar}
} % end small  

